From Aggregation to Selection: User-Validated Distributed Social Recommendation

Social recommender systems facilitate social connections by identifying potential friends for users. Each user maintains a local social network centered around themselves, resulting in a naturally distributed social structure. Recent research on distributed modeling for social recommender systems has gained increasing attention, as it naturally aligns with the user-centric structure of user interactions. Current distributed social recommender systems rely on automatically combining predictions from multiple models, often overlooking the user's active role in validating whether suggested connections are appropriate. Moreover, recommendation decisions are validated by individual users rather than derived from a single global ordering of candidates. As a result, standard ranking-based evaluation metrics make it difficult to evaluate whether a user-confirmed recommendation decision is actually correct. To address these limitations, we propose DeSocial, a distributed social recommendation framework with user-validation. DeSocial enables users to select recommendation algorithms to validate their potential connections, and the verification is processed through majority consensus among multiple independent user validators. To evaluate the distributed recommender system with user validator, we formulate this setting as a link prediction and verification task and introduce Acc@K, a consensus-based evaluation metric that measures whether user-approved recommendations are correct. Experiments on 4 real-world social networks shows that DeSocial improves decision correctness and robustness compared to single-point and distributed baselines. These findings highlight the potential of user-validated distributed recommender systems as a practical approach to social recommendation, with broader applicability to distributed and decentralized recommendations. Code: https://github.com/agiresearch/DeSocial.

==> table/alpha_sens.tex <==
\begin{table}[h]
\centering
\small
\renewcommand{\arraystretch}{0.9}
\setlength{\tabcolsep}{12pt}
\caption{Impact of time decay coefficient $\alpha$ on accuracy across datasets. Each block reports the means and the standard deviations (\%). Bold denotes the highest value per dataset at three evaluation metrics. All other parameters are fixed to their optimal values. }
\vspace{0.4cm}
\label{tab:alpha_sens}
\begin{tabular}{c|c|c|c|c}
\hline\hline
\rowcolor[HTML]{F0F0F0}
\textbf{Dataset} & \textbf{$\alpha$} & \textbf{Acc@2} & \textbf{Acc@3} & \textbf{Acc@5} \\ \hline
\multirow{4}{*}{\textbf{UCI}} & \textit{0} & 72.84 ± 0.27 & 62.38 ± 0.32 & 51.00 ± 0.33 \\
 & \textit{-0.01} & 73.02 ± 0.28 & 62.74 ± 0.32 & \textbf{51.37 ± 0.38} \\
 & \textit{-0.1} & \textbf{73.35 ± 0.28} & \textbf{62.80 ± 0.30} & 51.34 ± 0.32 \\
 & \textit{-1} & 72.35 ± 0.26 & 61.60 ± 0.31 & 49.94 ± 0.31 \\ \hline
\multirow{4}{*}{\textbf{Memo-Tx}} & \textit{0} & \textbf{83.96 ± 0.13} & \textbf{77.18 ± 0.14} & \textbf{69.31 ± 0.15} \\
 & \textit{-0.01} & 83.45 ± 0.13 & 76.72 ± 0.14 & 68.97 ± 0.14 \\
 & \textit{-0.1} & 83.37 ± 0.13 & 76.71 ± 0.14 & 69.07 ± 0.14 \\
 & \textit{-1} & 83.12 ± 0.11 & 76.60 ± 0.13 & 68.97 ± 0.13 \\ \hline
\multirow{4}{*}{\textbf{Enron}} & \textit{0} & 90.05 ± 0.09 & 85.94 ± 0.11 & \textbf{81.13 ± 0.13} \\
 & \textit{-0.01} & 90.02 ± 0.11 & 85.86 ± 0.13 & 80.92 ± 0.16 \\
 & \textit{-0.1} & \textbf{90.08 ± 0.11} & \textbf{85.96 ± 0.13} & 81.02 ± 0.17 \\
 & \textit{-1} & 89.60 ± 0.11 & 85.40 ± 0.13 & 80.39 ± 0.16 \\ \hline
\multirow{4}{*}{\textbf{GDELT}} & \textit{0} & 95.56 ± 0.02 & \textbf{92.44 ± 0.02} & 87.55 ± 0.04 \\
 & \textit{-0.01} & \textbf{95.57 ± 0.02} & \textbf{92.44 ± 0.02} & \textbf{87.58 ± 0.04} \\
 & \textit{-0.1} & 95.55 ± 0.02 & 92.40 ± 0.02 & 87.53 ± 0.04 \\
 & \textit{-1} & 95.48 ± 0.02 & 92.30 ± 0.02 & 87.36 ± 0.03 \\ \hline\hline
\end{tabular}
\end{table}

==> table/cost.tex <==
\begin{table}[ht]
\centering
\small
\caption{Estimated gas consumption for \model smart contract operations on Memo-Tx.}
\label{tab:cost}
\begin{tabular}{c|c|c|c}
\hline
\renewcommand{\arraystretch}{1}
\setlength{\arrayrulewidth}{0.75pt}
\textbf{Operation} & \# \textbf{of Ops.} & \textbf{Gas (Est.)} & \textbf{Total Est. Gas} \\
\hline
Link Validation     & 49706   & 20000  & 994120000 \\
Select Validators           & 49706   & 244000 & 12128264000 \\
Backbone Evaluation & 712      & 20000  & 14240000 \\
Vote                 & 248530  & 20000  & 4970600000 \\
Aggregate Decisions       & 10907   & 25800  & 281400600 \\
Broadcast                   & 10907   & 2100   & 22904700 \\
\hline
\textbf{Total}              &          &         & \textbf{18411529300} \\
\hline
\end{tabular}
\end{table}

==> table/f_sens.tex <==
\begin{table*}[ht]
\centering
\small
\renewcommand{\arraystretch}{1.25}
\setlength{\tabcolsep}{2.8pt}
\caption{Performance comparison over different  $\mathcal{F}$. Acc@2 (\%) is reported with mean and standard deviation. "Y" indicates improvement over all centralized models in $\mathcal{F}$, while "N" indicates not.}
\label{tab:f_sens}
\begin{tabular}{l|cc|cc|cc|cc}
\hline\hline
\rowcolor[HTML]{F0F0F0}
\multicolumn{1}{c|}{\textbf{$\mathcal{F}$}} & \multicolumn{2}{c|}{\textbf{UCI} } & \multicolumn{2}{c|}{\textbf{Memo-Tx}} & \multicolumn{2}{c|}{\textbf{Enron}} & \multicolumn{2}{c}{\textbf{GDELT}} \\
\cline{2-9}
\rowcolor[HTML]{F0F0F0}
& Acc@2 & $\uparrow$ & Acc@2 & $\uparrow$ & Acc@2 & $\uparrow$ & Acc@2 & $\uparrow$ \\
\hline
\textbf{MLP} & 66.38 $\pm$ 0.34 & - & 73.61 $\pm$ 0.11 & - & 81.48 $\pm$ 0.08 & - & 91.28 $\pm$ 0.02 & - \\
\textbf{GCN} & 63.90 $\pm$ 0.17 & - & 69.62 $\pm$ 0.13 & - & 79.92 $\pm$ 0.09 & - & 82.94 $\pm$ 0.04 & - \\
\textbf{GAT} & 61.15 $\pm$ 0.26 & - & 72.51 $\pm$ 0.26 & - & 85.52 $\pm$ 0.12 & - & 88.29 $\pm$ 0.28 & - \\
\textbf{SAGE} & 69.00 $\pm$ 0.40 & - & 82.85 $\pm$ 0.15 & - & 90.27 $\pm$ 0.06 & - & 93.16 $\pm$ 0.02 & - \\
\textbf{SGC} & 72.77 $\pm$ 0.24 & - & 80.37 $\pm$ 0.05 & - & 88.24 $\pm$ 0.04 & - & 95.59 $\pm$ 0.02 & - \\
\hline
\textbf{MLP+GCN} & 66.51 $\pm$ 0.23 & Y & 76.20 $\pm$ 0.10 & Y & 83.73 $\pm$ 0.09 & Y & 91.02 $\pm$ 0.02 & N \\
\textbf{MLP+GAT} & 65.73 $\pm$ 0.24 & Y & 74.22 $\pm$ 0.22 & Y & 86.57 $\pm$ 0.18 & Y & 91.36 $\pm$ 0.06 & Y \\
\textbf{MLP+SAGE} & 70.04 $\pm$ 0.39 & Y & 82.08 $\pm$ 0.16 & N & 89.86 $\pm$ 0.07 & N & 92.76 $\pm$ 0.02 & N \\
\textbf{MLP+SGC} & 73.19 $\pm$ 0.26 & Y & 80.73 $\pm$ 0.09 & Y & 88.29 $\pm$ 0.07 & Y & 95.42 $\pm$ 0.02 & N \\
\textbf{GCN+GAT} & 64.12 $\pm$ 0.27 & Y & 74.29 $\pm$ 0.24 & Y & 85.55 $\pm$ 0.17 & Y & 87.70 $\pm$ 0.16 & N \\
\textbf{GCN+SAGE} & 69.15 $\pm$ 0.39 & Y & 82.74 $\pm$ 0.16 & N & 89.88 $\pm$ 0.06 & N & 92.84 $\pm$ 0.02 & N \\
\textbf{GCN+SGC} & 72.74 $\pm$ 0.23 & N & 80.15 $\pm$ 0.08 & N & 88.24 $\pm$ 0.06 & N & 95.56 $\pm$ 0.02 & N \\
\textbf{GAT+SAGE} & 68.30 $\pm$ 0.44 & N & 81.83 $\pm$ 0.18 & N & 90.08 $\pm$ 0.11 & N & 92.96 $\pm$ 0.05 & N \\
\textbf{GAT+SGC} & 72.45 $\pm$ 0.23 & N & 78.42 $\pm$ 0.17 & N & 88.68 $\pm$ 0.07 & Y & 95.56 $\pm$ 0.02 & N \\
\textbf{SAGE+SGC} & 73.25 $\pm$ 0.33 & Y & 83.96 $\pm$ 0.13 & Y & 89.81 $\pm$ 0.04 & N & 95.57 $\pm$ 0.02 & N \\
\hline
\textbf{MLP+GCN+GAT} & 65.92 $\pm$ 0.26 & N & 75.45 $\pm$ 0.19 & Y & 86.22 $\pm$ 0.17 & Y & 91.29 $\pm$ 0.05 & Y \\
\textbf{MLP+GCN+SAGE} & 69.53 $\pm$ 0.33 & Y & 82.04 $\pm$ 0.12 & N & 89.66 $\pm$ 0.08 & N & 92.61 $\pm$ 0.02 & N \\
\textbf{MLP+GCN+SGC} & 72.79 $\pm$ 0.26 & Y & 80.60 $\pm$ 0.08 & Y & 88.17 $\pm$ 0.06 & N & 95.41 $\pm$ 0.02 & N \\
\textbf{MLP+GAT+SAGE} & 68.88 $\pm$ 0.34 & N & 81.08 $\pm$ 0.16 & N & 89.64 $\pm$ 0.10 & N & 92.74 $\pm$ 0.04 & N \\
\textbf{MLP+GAT+SGC} & 72.87 $\pm$ 0.27 & Y & 78.64 $\pm$ 0.15 & N & 88.62 $\pm$ 0.07 & Y & 95.40 $\pm$ 0.02 & N \\
\textbf{MLP+SAGE+SGC} & 73.25 $\pm$ 0.29 & Y & 83.57 $\pm$ 0.12 & Y & 89.79 $\pm$ 0.04 & N & 95.40 $\pm$ 0.02 & N \\
\textbf{GCN+GAT+SAGE} & 68.48 $\pm$ 0.37 & N & 81.73 $\pm$ 0.15 & N & 89.89 $\pm$ 0.09 & N & 92.82 $\pm$ 0.04 & N \\
\textbf{GCN+GAT+SGC} & 72.74 $\pm$ 0.22 & N & 78.20 $\pm$ 0.15 & N & 88.62 $\pm$ 0.07 & N & 95.55 $\pm$ 0.02 & N \\
\textbf{GCN+SAGE+SGC} & 72.98 $\pm$ 0.28 & Y & 83.79 $\pm$ 0.13 & Y & 89.71 $\pm$ 0.05 & N & 95.56 $\pm$ 0.02 & N \\
\textbf{GAT+SAGE+SGC} & 73.35 $\pm$ 0.27 & Y & 83.11 $\pm$ 0.15 & Y & 90.03 $\pm$ 0.06 & N & 95.55 $\pm$ 0.02 & N \\
\hline
\textbf{MLP+GCN+GAT+SAGE} & 69.03 $\pm$ 0.38 & Y & 81.20 $\pm$ 0.14 & N & 89.57 $\pm$ 0.11 & N & 92.64 $\pm$ 0.02 & N \\
\textbf{MLP+GCN+GAT+SGC} & 72.83 $\pm$ 0.28 & Y & 78.52 $\pm$ 0.17 & N & 88.70 $\pm$ 0.07 & Y & 95.40 $\pm$ 0.02 & N \\
\textbf{MLP+GCN+SAGE+SGC} & 73.35 $\pm$ 0.27 & Y & 83.27 $\pm$ 0.13 & Y & 89.57 $\pm$ 0.05 & N & 95.39 $\pm$ 0.02 & N \\
\textbf{MLP+GAT+SAGE+SGC} & 72.86 $\pm$ 0.26 & Y & 82.45 $\pm$ 0.16 & N & 89.77 $\pm$ 0.06 & N & 95.40 $\pm$ 0.02 & N \\
\textbf{GCN+GAT+SAGE+SGC} & 72.77 $\pm$ 0.30 & N & 82.63 $\pm$ 0.14 & N & 89.86 $\pm$ 0.07 & N & 95.54 $\pm$ 0.02 & N \\
\textbf{MLP+GCN+GAT+SAGE+SGC} & 73.07 $\pm$ 0.28 & Y & 82.36 $\pm$ 0.15 & N & 89.75 $\pm$ 0.06 & N & 95.39 $\pm$ 0.02 & N \\
\hline\hline
\end{tabular}
\end{table*}


==> table/gamma_sens.tex <==
\begin{table}[h]
\centering
\small
\renewcommand{\arraystretch}{0.9}
\setlength{\tabcolsep}{12pt}
\caption{Effect of neighbor sample size $\gamma$ on personalized algorithm selection performance (\%). Each block reports the means and the standard deviations. Best values per dataset are in bold.  All other parameters are fixed to their optimal values. }
\vspace{0.4cm}
\label{tab:gamma_sens}
\begin{tabular}{c|c|c|c|c}
\hline\hline
\rowcolor[HTML]{F0F0F0}
\textbf{Dataset} & \textbf{$\gamma$} & \textbf{Acc@2} & \textbf{Acc@3} & \textbf{Acc@5} \\
\hline
\multirow{5}{*}{\textbf{UCI}}
  & \textit{250}  & 73.15 ± 0.28 & 62.59 ± 0.29 & 51.02 ± 0.33 \\
  & \textit{500}  & 72.76 ± 0.24 & 62.33 ± 0.29 & 50.83 ± 0.30 \\
  & \textit{750}  & \textbf{73.35} ± 0.28 & \textbf{62.80} ± 0.30 & \textbf{51.34} ± 0.32 \\
  & \textit{1000} & 72.77 ± 0.29 & 62.26 ± 0.34 & 50.81 ± 0.37 \\
  & \textit{1250} & 72.44 ± 0.28 & 62.08 ± 0.31 & 50.74 ± 0.33 \\
\hline
\multirow{5}{*}{\textbf{Memo-Tx}}
  & \textit{250}  & 83.96 ± 0.13 & 77.18 ± 0.14 & 69.31 ± 0.15 \\
  & \textit{500}  & 83.81 ± 0.13 & 77.19 ± 0.14 & 69.52 ± 0.14 \\
  & \textit{750}  & 83.82 ± 0.12 & 77.03 ± 0.14 & 69.21 ± 0.15 \\
  & \textit{1000} & \textbf{83.91} ± 0.12 & \textbf{77.28} ± 0.12 & \textbf{69.57} ± 0.13 \\
  & \textit{1250} & 83.76 ± 0.14 & 76.97 ± 0.15 & 69.21 ± 0.17 \\
\hline
\multirow{5}{*}{\textbf{Enron}}
  & \textit{250}  & 89.63 ± 0.09 & 85.43 ± 0.12 & 80.40 ± 0.15 \\
  & \textit{500}  & 89.80 ± 0.09 & 85.65 ± 0.10 & 80.69 ± 0.12 \\
  & \textit{750}  & 89.98 ± 0.12 & 85.85 ± 0.14 & 80.88 ± 0.16 \\
  & \textit{1000} & 89.88 ± 0.10 & 85.75 ± 0.12 & 80.87 ± 0.15 \\
  & \textit{1250} & \textbf{90.08} ± 0.11 & \textbf{85.96} ± 0.13 & \textbf{81.02} ± 0.17 \\
\hline
\multirow{5}{*}{\textbf{GDELT}}
  & \textit{250}  & 95.54 ± 0.02 & 92.41 ± 0.03 & 87.54 ± 0.04 \\
  & \textit{500}  & 95.53 ± 0.02 & 92.40 ± 0.02 & 87.52 ± 0.04 \\
  & \textit{750}  & 95.54 ± 0.02 & 92.39 ± 0.02 & 87.51 ± 0.04 \\
  & \textit{1000} & \textbf{95.57} ± 0.02 & \textbf{92.44} ± 0.02 & \textbf{87.58} ± 0.04 \\
  & \textit{1250} & 95.55 ± 0.02 & 92.42 ± 0.02 & 87.55 ± 0.04 \\
\hline\hline
\end{tabular}
\end{table}


==> table/indus.tex <==
\begin{table*}[h]
%\large
\small
\centering
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1}
\caption{Comparison of Graphormer, Cluster-GCN, and \model on efficiency, scalability, privacy, and poising resilience. We denote the number of nodes and edges in the graph as $N$ and $E$ respectively. Let $L$ denote the number of GNN layers, $F$ the feature dimension, $b$ the batch size, and $\|A\|_0$ the number of non-zero entries in the adjacency matrix.}
\begin{tabular}{c|c|c|c|c|c}
\hline
\textbf{Framework} & \textbf{Time Complexity} & \textbf{Memory Complexity} & \textbf{Scalability} & \textbf{Privacy} & \textbf{Poisoning Resilience} \\
\hline
\textbf{Graphormer} & $\mathcal{O}(N^2 F)$ & $\mathcal{O}(N^2 + L F^2)$ & $\times$ & $\times$ & $\times$ \\
\textbf{Cluster-GCN} & $\mathcal{O}(L \|A\|_0 F + L N F^2)$ & $\mathcal{O}(b L F + L F^2)$ & $\checkmark$ & $\times$ & $\times$ \\
\textbf{\model} & $\mathcal{O}(L \|A\|_0 F + L N F^2)$ & $\mathcal{O}(L N F + L F^2)$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
\hline
\end{tabular}
\label{tab:industrial}

\end{table*}

==> table/run_time_both.tex <==
\begin{comment}
\begin{table*}[h]
\centering
\small
%\renewcommand{\arraystretch}{0.7}
\setlength{\tabcolsep}{7pt}
\caption{Run time (s) for each major step in \model under ETH Ganache simulation.}
\label{tab:runtime_both}
\begin{tabular}{c|c|c|c|c}
\hline
\textbf{Operation} & \textbf{Scale} & \textbf{Major Resource} & \textbf{UCI} & \textbf{Memo-Tx} \\ \hline
Validator Community Formation & $|\mathcal{E}^t|$ &  Smart Contract Execution & 0.1193 & 1.414 \\
Graph Model Training & $\mathcal{D}^t$ & Model Training (GPU) & 54.48 & 2011 \\
Create Backbone Evaluation Task & $|\mathcal{V}^t|$ & Python Random Function & 0.0022 & 0.0005 \\
Request on Backbone Evaluation & $|\mathcal{V}^t|$ & Smart Contract Execution & 0.0160 & 0.0177 \\
Evaluation Execution          & $|\mathcal{V}^t|$ & Model Inference & 0.0002 & 0.0002 \\
Return Evaluation Results & $|\mathcal{V}^t|$ &  Smart Contract Execution & 0.0161 & 0.0217 \\
Vote and Aggregation & $|\mathcal{E}^t|$ & Smart Contract Execution & 0.6233 & 9.081 \\
Merge Graph Data & $|\mathcal{V}|$ & Python Data Copy & 0.0249 & 0.2429 \\
\hline
\end{tabular}
\end{table*}
\end{comment}

\begin{table}[!t]
%\scriptsize
\small
\centering
\caption{Run time (unit: s; in 4 sig. figs.) and Acc@2 (\%) of \model and different baselines on UCI and Memo-Tx, given that all the models run for 100 epochs. Single refers to the single backbone baseline that reaches the best Acc@2 for UCI and Memo-Tx, reported in ~\autoref{tab:main_res}.}
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.9}
\label{tab:backbone-cost}
\begin{tabular}{c|c|c|c|c|c}
\hline
\textbf{Dataset} & \textbf{Single} & \textbf{GEN} & \textbf{E2GNN} & \textbf{FedGraphNN} & \textbf{\model} \\
\hline
\textbf{UCI Acc@2}     & 72.77 & 66.19 & 74.98 & 70.47 & \textbf{77.63} \\
\textbf{UCI Time}     & 46.43 & 48.52 & 77.45 & 24.88 & 107.9 \\
\hline
\textbf{Memo-Tx Acc@2} & 82.85  & 81.92 & 83.83 & 82.72 & \textbf{87.25} \\
\textbf{Memo-Tx Time}     & 2011  & 2015 & 2246 & 400.3 & 2637 \\
\hline
\end{tabular}
\end{table}



==> table/table_of_notation.tex <==
\begin{table}[h]
%\centering
\small
\begin{minipage}{\linewidth}
\raggedright
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{8pt}
\caption{List of main notations used in this paper.}
\label{tab:notation}
\begin{tabular}{l|l}
\hline\hline
\rowcolor[HTML]{F0F0F0}
\textbf{Symbol} & \textbf{Description} \\
\hline
$\mathcal{G}^t = (\mathcal{V}^t, \mathcal{E}^t)$ & Temporal graph at time $t$, with node set $\mathcal{V}^t$ and edge set $\mathcal{E}^t$ \\
$\mathcal{F}$ & Pool of backbone models. \\
$\mathcal{F}_{Full}$ & The set of backbones used in this paper, i.e., $\{\text{MLP}, \text{GCN}, \text{GAT}, \text{SAGE}, \text{SGC}\}$ \\
$f_{\Theta_u}$ & Graph learning model used by node $u$ with parameters $\Theta_u$ \\
$\Phi_{p,q,t}$ & Validator committee for verifying link $(p, q)$ at time $t$ \\
$Vote(\phi, p, q, t)$ & Binary decision by validator $\phi$ on link $(p, q)$ at time $t$ \\
$Ver(\Phi_{p,q,t}, p, q, t)$ & Aggregated verification result by majority voting over $\Phi_{p,q,t}$ \\
$\mathbf{z_u}$ & Embedding vector of node $u$ \\
$\sigma(\cdot)$ & Sigmoid activation function \\
$Neg(\phi, p, q, t)$ & Set of negative samples selected by validator $\phi \in \Phi_{p,q,t}$ \\
$\Gamma$ & Set of historical neighbor pairs $(v_p, v_n)$ for model selection \\
$\Pi_{u,v}$ & Temporal weight of edge $(u, v)$ based on its emergence time \\
$\mathcal{D}^t$ & All graph data up to time $t$, i.e., $\cup_{\tau=0}^t \mathcal{G}^{\tau}$ \\
$\mathcal{N}^t(u)$ & 1-hop neighbor set of $u$ in $\mathcal{G}^t$ \\
\hline\hline
\end{tabular}
\end{minipage}
\end{table}

